The pressure exerted by adsorbing directed lattice paths and staircase polygons

A directed path in the vicinity of a hard wall exerts pressure on the wall because of loss of entropy. The pressure at a particular point may be estimated by estimating the loss of entropy if the point is excluded from the path. In this paper we determine asymptotic expressions for the pressure on the X-axis in models of adsorbing directed paths in the first quadrant. Our models show that the pressure vanishes in the limit of long paths in the desorbed phase, but there is a non-zero pressure in the adsorbed phase. We determine asymptotic approximations of the pressure for finite length Dyck paths and directed paths, as well as for a model of adsorbing staircase polygons with both ends grafted to the X-axis.

==> figuregraph.tex <==
\beginpicture

 \setcoordinatesystem units <250.000 pt,150.000 pt>


 \color{blue}

\setplotsymbol ({\LARGE $\cdot$})


\plot 0 -1 0.5 0   /

 \color{black}
\put {O} at 0 0 
\setplotarea x from 0.000000 to 1.000000, y from -1.0000 to 0.00000
\axis bottom /
\axis right /
\axis left /
\axis top 
 label {{\Large \hspace{4cm} $a$}} /
\axis top 
 ticks out withvalues 0 0.5 1 / quantity 3 /
\axis left shiftedto x=0 
 label {{\Large $F_q^T$}} /
\axis left shiftedto x=0 
 ticks out withvalues -1 -0.75 {} -0.25 0  / quantity 5 /

\normalcolor
\endpicture

